Small-spatial scale variations of nebular properties and the abundance discrepancy in three Galactic HII regions

We present results of long-slit spectroscopy in several slit positions that cover different morphological structures of the central parts of three bright Galactic HII regions: M8, M17 and NGC7635. We study the spatial distributions of a large number of nebular parameters such as the extinction coefficient, line fluxes, physical conditions and ionic abundances at the maximum spatial resolution attainable with our instrumentation. Particularly, our goal is to study the behaviour of the abundance discrepancy factor of O^{2+}, ADF(O^{2+}), defined as the logarithmic difference of the O^{2+} abundances derived from collisionally excited and recombination lines. We find that the ADF(O^{2+}) remains fairly constant along the slit positions of M8 and M17. In the case of NGC7635, we only detect the OII recombination lines in the integrated spectrum along the whole slit, where the ADF(O^{2+}) reaches a remarkably high value of about 0.59 dex. We compare our results with previous ones obtained for the Orion Nebula. We find several evidences that suggest the presence of a candidate to Herbig-Haro object in M8.

==> tabla_ngctot.tex <==
        \multicolumn{2}{c}{K1}           & 9.00$\pm$0.20 & 7.58$\pm$0.11 & 8.42$\pm$0.09 & 6.86$\pm$0.14\\
        \multicolumn{2}{c}{K2}	         & 8.82$\pm$0.16 & 7.47$\pm$0.10 & 8.49$\pm$0.06 & 6.96$\pm$0.08\\
        \multicolumn{2}{c}{RIM}	         & 8.59$\pm$0.18 & 7.23$\pm$0.12 & 8.33$\pm$0.06 & 6.77$\pm$0.09\\        
\multirow{2}{*}{``Whole Slit"} & \tf$=0$ & 8.88$\pm$0.13 & 7.49$\pm$0.10 & 8.40$\pm$0.08 & 6.87$\pm$0.08\\  			      
                               & \tf$>0$ & 8.66$\pm$0.13 & 7.98$\pm$0.17 & 8.76$\pm$0.09 & 7.46$\pm$0.11\\
\hline			       
\multicolumn{2}{c}{\cite{shaveretal83}}     &     --      & 7.67$\pm$0.15 & 8.81$\pm$0.15 &       --     \\ 
\multicolumn{2}{c}{\cite{afflerbachetal97}} &     --      & 7.76$\pm$0.08 & 8.56$\pm$0.11 & 6.67$\pm$0.07\\  
\multicolumn{2}{c}{\cite{deharvengetal00}}  &     --      &       --      & 8.46$\pm$0.07 &       --     \\   
\multicolumn{2}{c}{\cite{estebanetal05}}  & 8.45$\pm$0.20 &       --      & 8.64$\pm$0.12 &       --     \\ 
			       
			       
			       
			       

